Generative Adversarial Networks (GAN) Powered Fast Magnetic Resonance Imaging -- Mini Review, Comparison and Perspectives

Magnetic Resonance Imaging (MRI) is a vital component of medical imaging. When compared to other image modalities, it has advantages such as the absence of radiation, superior soft tissue contrast, and complementary multiple sequence information. However, one drawback of MRI is its comparatively slow scanning and reconstruction compared to other image modalities, limiting its usage in some clinical applications when imaging time is critical. Traditional compressive sensing based MRI (CS-MRI) reconstruction can speed up MRI acquisition, but suffers from a long iterative process and noise-induced artefacts. Recently, Deep Neural Networks (DNNs) have been used in sparse MRI reconstruction models to recreate relatively high-quality images from heavily undersampled k-space data, allowing for much faster MRI scanning. However, there are still some hurdles to tackle. For example, directly training DNNs based on L1/L2 distance to the target fully sampled images could result in blurry reconstruction because L1/L2 loss can only enforce overall image or patch similarity and does not take into account local information such as anatomical sharpness. It is also hard to preserve fine image details while maintaining a natural appearance. More recently, Generative Adversarial Networks (GAN) based methods are proposed to solve fast MRI with enhanced image perceptual quality. The encoder obtains a latent space for the undersampling image, and the image is reconstructed by the decoder using the GAN loss. In this chapter, we review the GAN powered fast MRI methods with a comparative study on various anatomical datasets to demonstrate the generalisability and robustness of this kind of fast MRI while providing future perspectives.

==> GAN Powered Fast MRI/sections/CNN_MRI_recon.tex <==
CNN excels in computer vision applications compared to traditional machine learning methods in general, and has been increasingly incorporated into CS-based MRI reconstruction models. It achieves higher accuracy and acceleration of MRI acquisition compared to traditional CS models \cite{Yang2018,Eo2018,Schlemper2018,qin_convolutional_2019}. A CNN consists of a series of convolutional layers connected by non-linear activation functions \cite{jogin_feature_2018}. In each convolutional layer, multiple filters are convolved with the input image or the output from a previous layer to extract image specific features \cite{jogin_feature_2018}. The weight of each filter is optimised such that the final reconstructed image matches the original fully sampled image. By stacking multiple convolutional layers, the large number of weight parameters in a CNN endows it with the potential to model complex functions, including recovering the fully sampled images from the undersampled ones.

The process of optimising the weights of CNN is known as training the network and is governed by an optimisation objective called the loss function. The loss functions differ between supervised and unsupervised settings, depending on whether fully sampled ground truth images are available. In a supervised learning setting, fully sampled images are used to ``teach'' the CNN model to minimise the loss, or difference, between the reconstructed results and the fully sampled ground truth. However, in an unsupervised environment, ground truth images are not available, meaning the loss function can be, for example, optimised based on the Deep Image Prior framework and uses a high-resolution reference MR image as the input of the CNN to induce the structural prior in the learning procedure \cite{zhao_reference-driven_2020}. Unsupervised CNN-based CS-MRI models are beyond the scope of this chapter, which will instead focus on the supervised learning models.

Supervised CNN-based CS-MRI methods can be broadly divided into two categories: end-to-end and unrolled optimisation \cite{liang_deep_2019,liang_deep_2020,zhang_review_2020}.  End-to-end methods model the inverse of the acquisition process (Eq \ref{eq:CS_acquisition}) by mapping the undersampled input to the reconstructed output directly, hence the name ``end-to-end'':
\begin{equation}
    \hat x_u = f_{\mathrm{CNN}} (y_u|\theta),
\end{equation}
where $f_{CNN}$ is the operation performed by the CNN and $\theta$ represents all the parameters within the CNN. The $\theta$ is optimised by minimising the difference between $\hat x_u$ and the ground truth $x_t$.  Such end-to-end techniques are exemplified by U-Net \cite{lee_deep_2018} and generative adversarial network (GAN) \cite{Yang2018,Mardani2019,Quan2018}. 

In contrast, CNN-based unrolled optimisation methods perform iterative image update based upon the general CS reconstruction model (Eq \ref{eq:CS_eq}). Unlike non-CNN based CS techniques, where the term $R(\hat x_u)$ is an expert-designed regularisation function, the CNN-based unrolled methods apply CNN to learn the optimal way of regularising an image. This is exemplified by the deep cascade CNN (DC-CNN) network \cite{Schlemper2018}, whose regulariser term penalises the deviation of the reconstructed image from the CNN output:
\begin{equation}
    \argmin_{\hat x_u, \theta} \frac{\lambda}{2}||y_u-A \hat x_u||_2^2 + ||\hat x_u-f_{\mathrm{CNN}}(y_u|\theta)||.
\label{eq:CNN_DCCNN}\end{equation}

Another example is the variational network \cite{Hammernik2018}, which uses a Field-of-Expert regularisation function:

\begin{equation}
    \argmin_{\hat x_u, \theta} \frac{\lambda}{2}||y_u-A\hat x_u||_2^2 + \sum_i f_i(k_i\hat x_u),
\label{eq:CNN_VN}\end{equation}
where $f_i$ is a learnable activation function and $k_i$ represents a convolutional filter. From a Bayesian point of view, these CNN-based regularisers form the prior expectation of the reconstructed images by learning from the ground truth MR
images.

While both end-to-end and unrolled methods can incorporate CNN to learn the image reconstruction or regularisation process, a key difference between them is that unrolled methods need to iteratively update the images during the reconstruction process. In contrast, end-to-end ones compute the output directly. 
Hence, it is more time consuming to train unrolled CNN-based models and to apply them in reconstruction, compared with end-to-end methods, with other comparisons summarised in Table \ref{tab:UO_ETE}.  This suggests an advantage of developing end-to-end methods, such as GAN-based models, for CS-MRI reconstruction.

\begin{table}
\begin{center}
\begin{tabular}{lll}
        \toprule
        \textbf{Category} & \textbf{End-to-end} & \textbf{Unrolled} \\
        \midrule
        Reconstruction time & Short & Long  \\
        Data fidelity & No    & Yes  \\
        Sample size   & Larger & Smaller\\
        Performance   & Lower & Higher\\
        Weight update & Yes   & Yes  \\
        Image update  & No    & Yes  \\
        Parameter number & Larger & Smaller \\
        \bottomrule
\end{tabular}
\end{center}
\caption{Comparison between end-to-end and unrolled optimisation methods in
        CNN-based CS-MRI models \cite{liang_deep_2019,liang_deep_2020,zhang_review_2020}.}
\label{tab:UO_ETE}\end{table}


==> GAN Powered Fast MRI/sections/Method_DAGAN.tex <==
Deep De-Aliasing Generative Adversarial Networks (DAGAN) was proposed in 2017 by Yang et al. \cite{Yang2018,yu2017deep} for fast compressed sensing MRI reconstruction. Figure \ref{dagan} shows the architecture of DAGAN.

As shown in Figure \ref{dagan_generator}, a modified U-Net \cite{Ronneberger2015} was used as the generator $G$, which consisted of 8 convolutional layers in the encoding path and 8 deconvolutional layers in the decoding path. The stride of all convolutional and deconvolutional layers was set to 2 for downsampling and upsampling the feature maps. Each convolutional layer was followed by a Batch Normalisation (BN) layer and a Leaky ReLU (LReLU) layer. Skip connection was applied between corresponding layers in the encoding and decoding paths in order to pass the features in the encoding layer to the decoding layer for better reconstruction details. The modified U-Net ended up with a hyperbolic tangent function as the activation function. Due to the alternating training strategy in the adversarial components, the original GAN model is hard to train. DAGAN applied $\hat x_u=G(x_u)+x_u$ instead of $\hat x_u=G(x_u)$ as the output of the generator for better stability and faster convergence speed. In this way, DAGAN turned the generator into a refinement function, which means that it only generated the missing information, and the complexity of the model was reduced.

As shown in Figure \ref{dagan_discriminator}, an 11-layer CNN architecture was used as the discriminator $D$. A BN layer and a LReLU layer were followed with each convolutional layer. Finally, a full connection (FC) layer was cascaded, and the classification result was output through the Sigmoid activation function. 

In DAGAN, normalised MSE was used as the optimisation cost function. However, only optimising the pixel-wise MSE loss in the image domain could result in non-smooth reconstructions, which might lack coherent image details. To solve this problem, a data consistency loss was designed for training the generator in both frequency and image domains to help the optimisation and to exploit the complementary properties of the two domains. Besides, perceptual similarity \cite{Ledig_2017_CVPR} was also incorporated. In so doing, the data consistency loss consists of three parts: pixel-wise image domain MSE loss $L_{\mathrm{iMSE}}$, frequency domain MSE loss $L_{\mathrm{fMSE}}$, and the pre-trained VGG perceptual loss $L_{\mathrm{VGG}}$ \cite{simonyan2015deep}. They can be defined as:

\begin{equation}
L_{\mathrm{iMSE}}(\theta_G) =
\frac{1}{2}\mid\mid x_t -  \hat x_u \mid\mid^2_2,
\end{equation}

\begin{equation}
L_{\mathrm{fMSE}}(\theta_G) =
\frac{1}{2}\mid\mid \mathcal{F} x_t- \mathcal{F} \hat x_u \mid\mid^2_2,
\end{equation}

\begin{equation}
L_{\mathrm{VGG}}(\theta_G) =
\frac{1}{2}\mid\mid f_{\mathrm{VGG}}(x_t) - f_{\mathrm{VGG}}(\hat x_u) \mid\mid^2_2.
\end{equation}

Here, $\mid\mid\cdot\mid\mid^2_2$ denotes the L2 norm, $f_{\mathrm{VGG}}(\cdot)$ denotes VGG network (the Conv4 output of the VGG16), and was pretrained on the ImageNet \cite{RussakovskyDeng-363}.

The adversarial loss $L$ can be defined as:
\begin{dmath}
L_{\mathrm{adv}}(\theta_G, \theta_D)
=\mathbb{E}_{{x_t} \sim P_{\mathrm{train}}(x_t)}
[\mathop{\text{log}} D_{\theta_D}({x_t})] ~\\
+\mathbb{E}_{{x_u} \sim p_{G}(x_u)}
[\mathop{\text{log}} (1-D_{\theta_D}(G_{\theta_G}(x_u))],
\end{dmath}
where $P_{\mathrm{train}}(x_t)$ denotes the collection of MR image ground truth, and $p_{G}(x_u)$ denotes the collection of MR image reconstruction.

Therefore the total loss function can be represented as:
\begin{dmath}
L_{\mathrm{TOTAL}}(\theta_G, \theta_D)
= \alpha L_{\mathrm{iMSE}}(\theta_G)
+ \beta L_{\mathrm{fMSE}}(\theta_G)
+ \gamma L_{\mathrm{VGG}}(\theta_G) ~\\
+ L_{\mathrm{adv}}(\theta_G, \theta_D),
\end{dmath}
where $\alpha$, $\beta$ and $\gamma$ were the weights of different components of the loss function, which balanced different loss terms into similar scales according to previous study. Here, $\alpha=15$, $\beta=0.1$ and $\gamma=0.0025$ were set empirically, according to the original paper.

\begin{figure}[!h]
\centering\includegraphics[width=5in]{DAGAN/DAGAN.pdf}
\caption{The architecture of DAGAN. The generator produced the MR image $\hat x_u$ from the undersampled MR image. The generated MR image $\hat x_u$ and the ground truth MR image were input into the discriminator for adversarial loss $L_{\mathrm{adv}}$ calculation. The data consistency loss consisted of image domain MSE loss $L_{\mathrm{iMSE}}$, frequency domain MSE loss $L_{\mathrm{fMSE}}$, and VGG perceptual loss $L_{\mathrm{VGG}}$.}
\label{dagan}
\end{figure}

\begin{figure}[!h]
\centering\includegraphics[width=5in]{DAGAN/DAGAN_generator.pdf}
\caption{Structure of the generator in DAGAN. The generator was based on a modified U-Net, which consisted of 8 convolutional layers and 8 transposed convolutional layers (de-convolutional layers), with a BN layer and a LReLU or ReLu layer followed with each layer. Skip connection between layers that were the same scale and shortcut connections between the input and output of the generator were applied. A hyperbolic tangent function was used as an output activation function. (C: Convolutional layer; DC: De-Convolutional layer; B: Batch Normalization layer; L: Leaky ReLU layer; R: ReLU layer; T: hyperbolic tangent function.)}
\label{dagan_generator}
\end{figure}

\begin{figure}[!h]
\centering\includegraphics[width=5in]{DAGAN/DAGAN_discriminator.pdf}
\caption{Structure of the discriminator in DAGAN. Essentially, the discriminator was an 11-layer CNN classifier. Each convolutional layer was cascaded by a BN layer and a LReLu Layer. A full connection layer and a Sigmoid function were applied to output the result of the classification. (C: Convolutional layer; B: Batch Normalization layer; L: Leaky ReLU layer; F: Full Connection layer; S: Sigmoid function.)}
\label{dagan_discriminator}
\end{figure}

==> GAN Powered Fast MRI/sections/Method_GAN.tex <==
Inspired by the two-player zero-sum game in game theory, GAN \cite{Goodfellow2014} consists of two players: a generator and a discriminator. Traditionally, the generator $G$ captures the distribution of sample data, and uses noise $z$ that follows a certain distribution to generate a sample $G(z)$ similar to the real training data $x_t$. The discriminator $D$ is a binary classifier, which aims to distinguish fake data generated by $G$ from the ground truth. If the sample comes from the real training data, $D$ outputs a large probability, otherwise, $D$ outputs a small probability. Ideally, the best $D$ can be represented as $D(x_t)=1$ and $D(G(z))=0$. In this way, the generator and the discriminator form a min-max game. The training process of GAN can be described as follows:

\begin{dmath}
\mathop{\text{min}}\limits_{\theta_G} \mathop{\text{max}}\limits_{\theta_D}
L(\theta_G, \theta_D)
=\mathbb{E}_{\bm{x} \sim p_{\mathrm{data}}(\bm{x})}
[\mathop{\text{log}} D_{\theta_D}(\bm{x})] ~\\
+\mathbb{E}_{\bm{z} \sim p_{\bm{z}}(\bm{z})}
[\mathop{\text{log}} (1-D_{\theta_D}(G_{\theta_G}(\bm{z}))],
\end{dmath}
where $p_{\mathrm{data}}(\bm{x})$ is the distribution of the training dataset, and the $p_{\bm{z}}(\bm{z})$ is the distribution of the latent variables. 

Alternating gradient optimisation between $G$ and $D$ is used to train the GAN. In this process, both models try their best to optimise their networks to form a competitive confrontation until the two models reach a dynamic balance. Ideally, the final result is that the image generated by $G$ is very similar to the real image, and it is difficult for the $D$ network to distinguish between the real image and the image generated by $G$, i.e., $D(G(Z)) = 0.5$.




==> GAN Powered Fast MRI/sections/Method_KIGAN.tex <==
KIGAN was introduced by Shaul et al. \cite{SHAUL2020101747}. The overall structure of KIGAN is shown in Figure \ref{kigan}. A \textit{k}-space generator $G_{\mathrm{K}}$ and an image space generator $G_{\mathrm{IM}}$ were cascaded in KIGAN. Adjacent undersampled \textit{k}-space slices (along the third dimension or the temporal dimension) $y^{l-1}_u$, $y^{l}_u$ and $y^{l+1}_u$ were the input of $G_{\mathrm{K}}$. A data consistency step, i.e., $\widetilde{y}_u=\bar{\Psi} G_{\mathrm{K}}(y^{l-1}_u,y^{l}_u,y^{l+1}_u) + y^{l}_u$ was applied for merging the output with the reconstructed missing data. $G_{\mathrm{IM}}$ was able to generate the output of $G_{\mathrm{K}}$ in image space, i.e., $\widetilde{x}_u$, to reconstructed image $\hat{x}_u$. Refinement learning $\hat{x}_u=G_{\mathrm{IM}}(\widetilde{x}_u)+\widetilde{x}_u$ was also used as the output of $G_{\mathrm{IM}}$ instead of $\hat{x}_u=G_{\mathrm{IM}}(\widetilde{x}_u)$. The reconstruction MR image $\hat{x}_u$, together with MR ground truth image $x_t$ were sent to the discriminator for the adversarial loss.

As shown in Figures \ref{kigan_generator_K} and \ref{kigan_generator_i}, the main structure of the generators $G_{\mathrm{K}}$ and $G_{\mathrm{IM}}$ were based on a modified U-Net, which consisted of 5 convolutional layers in the encoding path and 5 deconvolutional layers in the decoding path, where each convolutional and deconvolutional layer were followed by a BN layer and a LReLU layer. Skip connection was applied between corresponding layers in the encoding and decoding paths, in order to pass the feature of different scales to the decoding layer for better reconstruction details. Additionally, in $G_{\mathrm{IM}}$, a shortcut connection between the input and output was applied for turning $G_{\mathrm{IM}}$ into a refinement function. 

As shown in Figure \ref{kigan_discriminator}, the discriminator was a standard 9-layer CNN structure with an FC layer and a Sigmoid activation function connected for the result of the classification. 

The loss function of KIGAN consisted of: an image domain MSE loss $L_{\mathrm{iMSE}}$, a frequency domain MSE loss $L_{\mathrm{fMSE}}$, and an adversarial loss $L_{\mathrm{adv}}$, which can be defined as:
\begin{equation}
L_{\mathrm{iMSE}}(\theta_{\mathrm{K}}, \theta_{\mathrm{IM}}) 
=\frac{1}{2}\mid\mid x_t -  \hat x_u \mid\mid^2_2,
\end{equation}

\begin{equation}
L_{\mathrm{fMSE}}(\theta_{\mathrm{K}}) 
=\frac{1}{2}\mid\mid y^l_t- \widetilde y_u \mid\mid^2_2,
\end{equation}

\begin{equation}
L_{\mathrm{adv}}(\theta_{\mathrm{K}}, \theta_{\mathrm{IM}}, \theta_D)
=\mathbb{E}_{x_t \sim M}
[\mathop{\text{log}} D_{\theta_D}(x_t)]
+\mathbb{E}_{\hat x_u \sim S}
[\mathop{\text{log}} (1-D_{\theta_D}(\hat x_u)],
\end{equation}
where $M$ denotes the collection of image space ground truth, and $S$ denotes the collection of image space reconstruction.

The whole loss function can be represented as:
\begin{dmath}
L_{\mathrm{TOTAL}}(\theta_{\mathrm{K}}, \theta_{\mathrm{IM}}, \theta_D) 
= \alpha L_{\mathrm{iMSE}}(\theta_{\mathrm{K}}, \theta_{\mathrm{IM}}) 
+ \beta L_{\mathrm{fMSE}}(\theta_{\mathrm{K}}) ~\\
+ L_{\mathrm{adv}}(\theta_{\mathrm{K}}, \theta_{\mathrm{IM}}, \theta_D), 
\end{dmath}
where $\alpha$, $\beta$ are the hyperparameters that control the balance of different components in the loss function. 


\begin{figure}[!h]
\centering\includegraphics[width=5in]{KIGAN/KIGAN.pdf}
\caption{The Architecture of KIGAN. Two generators and one discriminator were used in KIGAN. \textit{k}-space generator was able to reconstruct \textit{k}-space MR data $G_{\mathrm{K}}(y^{l}_u)$ from a cascade of undersampled \textit{k}-space MR data $y^{l-1}_u$, $y^{l}_u$ and $y^{l+1}_u$, and image space generator was able to reconstruct the MR image $\hat x_u$ (final result). The discriminator was to output the classification result of ground truth MR image $x_t$ and generated MR image $\hat x_u$ for adversarial loss $L_{\mathrm{loss}}$. Image domain MSE loss $L_{\mathrm{iMSE}}$ and frequency domain MSE loss were added into the total loss function.}
\label{kigan}
\end{figure}

\begin{figure}[!h]
\centering\includegraphics[width=5in]{KIGAN/KIGAN_generator_K.pdf}
\caption{The Structure of \textit{k}-space Generator in KIGAN. Five convolutional layers and five de-convolutional layers were applied as encoding path and decoding path in the generator respectively. A convolutional layer was used as the output layer to adjust the channel of the reconstructed MR image. Corresponding layers of the same scales were linked by the skip connection. (C: Convolutional layer; DC: De-Convolutional layer; B: Batch Normalization layer; L: Leaky ReLU layer; R: ReLU layer.)
}
\label{kigan_generator_K}
\end{figure}

\begin{figure}[!h]
\centering\includegraphics[width=5in]{KIGAN/KIGAN_generator_I.pdf}
\caption{The Structure of image space Generator in KIGAN. 5 convolutional layers and 5 de-convolutional layers were applied as encoding path and decoding path in the generator respectively. A convolutional layer and a hyperbolic tangent function were used as the output layer. Skip connection and shortcut connection were adopted in the image space generator. (C: Convolutional layer; DC: De-Convolutional layer; B: Batch Normalization layer; L: Leaky ReLU layer; R: ReLU layer; T: hyperbolic tangent function.)
}
\label{kigan_generator_i}
\end{figure}

\begin{figure}[!h]
\centering\includegraphics[width=5in]{KIGAN/KIGAN_discriminator.pdf}
\caption{The Structure of Discriminator in KIGAN. The discriminator was a standard 9-layer CNN structure with an FC layer and a Sigmoid activation function connected for the result of the classification. (C: Convolutional layer; B: Batch Normalization layer; L: Leaky ReLU layer; F: Full Connection layer; S: Sigmoid function.)}
\label{kigan_discriminator}
\end{figure}

==> GAN Powered Fast MRI/sections/Method_ReconRefineGAN.tex <==
ReconGAN/RefineGAN was proposed by Quan et al. \cite{Quan2018} for compressed sensing MRI reconstruction. Figure \ref{reconrefinegan} shows the architecture of ReconGAN/RefineGAN. The two-fold chained network that consisted of 2 U-shaped generators ($G_1$ and $G_2$ respectively) was able to generate a 2-channel zero-filling MR image (real part and imaginary part) directly into a 2-channel reconstructed MR image. The checkpoints after $G_1$ and $G_2$ were defined as ReconGAN and RefineGAN respectively.

As shown in Figure \ref{reconrefinegan_generator}, the generator consisted of 4 encoder blocks in the encoding path and 4 decoder blocks in the decoding path. Skip connection between corresponding blocks that had the same scale was adopted to pass the feature from the encoding path to the decoding path. $\bar x_u=G_1(x_u)+x_u$ and $\hat x_u=G_2(\bar x_u)+\bar x_u$ were used as the output of the generator instead of $\bar x_u=G_1(x_u)$ and $\hat x_u=G_2(\bar x_u)$ for better reconstruction details and faster convergence speed. Figures \ref{reconrefinegan_encoder} and \ref{reconrefinegan_decoder} show the structure of the encoder block and decoder block. The encoder block consisted of 2 convolutional layers and a residual block inserted between them. The stride of the first convolutional layer was set to 2 for the downsampling. The decoder block consisted of 2 transposed convolutional layers and a residual block inserted between them. The stride of the second transposed convolutional layer was set to 2 for upsampling. 
The residual block consisted of three convolutional layers, the kernel number in the second convolutional layer was half of the kernel number in the first and third convolutional layer. A shortcut connection was linked between the input and output of the residual block.

As shown in Figure \ref{reconrefinegan_discriminator}, the encoding path in the generator was adopted as the main structure of the discriminator. An FC layer and Sigmoid function were cascaded after the encoding path for the classification result.

The loss function of ReconGAN/RefineGAN was consisted of: image domain MSE loss $L_{\mathrm{iMSE}}$, frequency domain MSE loss $L_{\mathrm{fMSE}}$, and the adversarial loss $L_{\mathrm{adv}}$, which can be defined as:

\begin{equation}
L_{\mathrm{iMSE}}(\theta_{G_1}, \theta_{G_2}) =
\frac{1}{2}\mid\mid x_t -  \hat x_u \mid\mid^2_2,
\end{equation}

\begin{equation}
L_{\mathrm{fMSE}}(\theta_{G_1}, \theta_{G_2}) =
\frac{1}{2}\mid\mid \mathcal{F} x_t- \mathcal{F} \hat x_u \mid\mid^2_2,
\end{equation}

\begin{dmath}
L_{\mathrm{adv}}(\theta_{G_1}, \theta_{G_2}, \theta_D)
=\mathbb{E}_{{x_t} \sim P_{train}(x_t)}
[\mathop{\text{log}} D_{\theta_D}({x_t})]
+\mathbb{E}_{{x_u} \sim p_{G_2G_1}(x_u)}
[\mathop{\text{log}} (1-D_{\theta_D}(G_{\theta_{G_2}}(G_{\theta_{G_1}}(x_u)))].
\end{dmath}

The total loss function can be represented as:

\begin{dmath}
L_{\mathrm{TOTAL}}(\theta_{G_1}, \theta_{G_2}, \theta_D)
= \alpha L_{\mathrm{iMSE}}(\theta_{G_1}, \theta_{G_2})
+ \beta L_{\mathrm{fMSE}}(\theta_{G_1}, \theta_{G_2})
+ L_{\mathrm{adv}}(\theta_{G_1}, \theta_{G_2}, \theta_D),
\end{dmath}
where $\alpha=10$, $\beta=0.1$ were the hyperparameters that controlled the balance of different components in the loss function. 

\begin{figure}[!h]
\centering\includegraphics[width=5in]{ReconRefineGAN/RefineGAN.pdf}
\caption{The architecture of ReconGAN/RefineGAN. A two-fold chained network with 2 generators cascaded was used as the generator to produce reconstructed MR images $\hat x_u$ from undersampled MR images $x_u$. Reconstructed MR images $\hat x_u$ together with ground truth MR images $x_t$ were sent to the discriminator for the calculation of the adversarial loss $L_{\mathrm{adv}}$. Besides, image domain MSE loss $L_{\mathrm{iMSE}}$ and frequency domain MSE loss $L_{\mathrm{fMSE}}$ were added to the total loss function for training the generator.}
\label{reconrefinegan}
\end{figure}

\begin{figure}[!h]
\centering\includegraphics[width=5in]{ReconRefineGAN/RefineGAN_generator.pdf}
\caption{Structure of the generator in ReconGAN/RefineGAN. The generator consisted of 4 encoder blocks in the encoding path and 4 decoder blocks in the decoding path. Skip connection was linked between blocks of the same scale in different paths. A shortcut connection was applied between the input and output of the generator, which turns the generator into a refinement function. (EB: Encoder Block; DB: Decoder Block.)
}
\label{reconrefinegan_generator}
\end{figure}

\begin{figure}[!h]
\centering\includegraphics[width=3in]{ReconRefineGAN/RefineGAN_encoder_block.pdf}
\caption{Structure of the encoder block in the generator of ReconGAN/RefineGAN. (C: Convolutional layer; B: Batch Normalization layer; L: Leaky ReLU layer.)}
\label{reconrefinegan_encoder}
\end{figure}

\begin{figure}[!h]
\centering\includegraphics[width=3in]{ReconRefineGAN/RefineGAN_decoder_block.pdf}
\caption{Structure of the decoder block in the generator of ReconGAN/RefineGAN. (C: Convolutional layer; DC: De-Convolutional layer; B: Batch Normalization layer; L: Leaky ReLU layer.)}
\label{reconrefinegan_decoder}
\end{figure}

\begin{figure}[!h]
\centering\includegraphics[width=3in]{ReconRefineGAN/RefineGAN_discriminator.pdf}
\caption{Structure of the discriminator in ReconGAN/RefineGAN. The main structure adopted the encoding path of the generator. A full connection layer and a Sigmoid activation function were cascaded at the end of the discriminator. (C: Convolutional layer; L: Leaky ReLU layer; F: Full Connection layer; S: Sigmoid function; EB: Encoder Block.)}
\label{reconrefinegan_discriminator}
\end{figure}


==> GAN Powered Fast MRI/sections/discussion.tex <==
We have established that GAN based methods such as DAGAN, KIGAN, ReconGAN, and RefineGAN excel in generating faithful, photo-realistic reconstruction of undersampled MR images and in removing the undersampling artefacts.  Despite their representing a successful category of CS-MRI techniques, GAN based methods suffer from training instability and slow convergence to a global minimum \cite{Chen2017,Wiatrak2020}. This problem can be alleviated by Wasserstein GAN (WGAN) \cite{Arjovsky2017}.  Instead of minimising Jensen-Shannon divergence between the reconstructed image and ground truth in the training phase, WGAN aims to reduce the Wasserstein distance.  WGAN based CS-MRI models have achieved superior reconstruction performance compared with GAN based methods e.g., DAGAN \cite{jiang_accelerating_2019,oh_unpaired_2020}. However, to minimise the Wasserstein distance, the discriminator needs to satisfy the 1-Lipschitz constraint. The original WGAN paper adopted a weight clipping approach to enforce this constraint but this can itself cause training instability. The potential improvement includes a gradient clipping approach \cite{Gulrajani2017} or dividing the weights of neural networks by their spectral norm \cite{miyato_spectral_2018}. Altogether, modifying the loss function of GAN is key to addressing its training instability issue.

Another problem with the GAN loss function is that it may affect the high frequency texture \cite{Mardani2019} and smoothing the reconstructed image \cite{zhao_loss_2017}. GAN may also generate high frequency noise \cite{Mardani2019}. Mardani et al. (2019) suggested solving the high frequency texture issue with the least square GAN \cite{Mardani2019}. L1 loss between reconstructed images and ground truth was also added as an auxiliary function, to serve as a low-pass filter to remove high frequency noises.

Apart from the issues with the GAN loss function during training, GAN based methods suffer from reconstruction instability \cite{antun_instabilities_2020}. This means that a small perturbation to the input image leads to large scale changes in the reconstruction output.  Antun et al. (2020) \cite{antun_instabilities_2020} evaluated the instabilities of DAGAN and other deep learning based CS-MRI models and showed that the performance of DAGAN deteriorated as the undersampling ratio increased during testing. That is if more \textit{k}-space pixels were undersampled more than the undersampling ratio in the images used to train DAGAN, its performance decreases. In contrast, variational network and deep cascaded convolutional neural networks (DC-CNN), two non-GAN based techniques, did not experience the same issue.  This indicates the incorporation of GAN may reduce the generalisability of the model to images collected under different undersampling ratios and contribute to its reconstruction instability.

Another instability issue with DAGAN is that if small structural details were added to an MRI image, such as random letters, and this image was undersampled retrospectively, DAGAN was unable to reconstruct the structural details. In contrast, variational network and DC-CNN were superior in recovering these structural details \cite{antun_instabilities_2020}. Even though these two instability tests revealed a critical weakness of DAGAN, DAGAN, being one of the earliest GAN based methods, may not capture the improved reconstruction accuracy and network architectural complexity of the more recent methods \cite{jiang_accelerating_2019,oh_unpaired_2020}. Hence, more instability testing is required on more GAN based methods to conclude whether this category of CS-MRI techniques suffers from reconstruction instability.

These results on instability testing still question the generalisability of GAN based models. In other words, it is unclear whether after being trained with images from one  source, e.g., one organ, under one undersampling ratio etc, a model will achieve equivalent performance on images from another source. This is often referred to in the literature as a zero-shot inference test. However, GAN based methods appear to excel in these inference tests. To illustrate, DAGAN, having been trained with MR images of the brain of a healthy volunteer, successfully reconstructed the MR images from a patient with the brain tumour, faithfully preserving the tumour structure \cite{Yang2018}. Another example is that GANCS, another GAN based method, was trained with MR images of the abdomen and any images containing the enlarged adrenal gland were removed from the training set. In testing, GANCS was capable of recovering enlarged adrenal gland in patients with adrenal hypertrophy. No evidence of hallucination of the reconstructed images was found \cite{Mardani2019}. These successes in the zero-shot inference of pathological structures challenged the instability test results from Antun et al. One interpretation is that the additional structural details added to the MR images by Antun et al., such as letters, may not represent real-life physiological or pathological deviations of the MR images from the training set. It was also possible that the zero-shot inference tests on DAGAN and GANCS concerned only a small sample size, limited to a few pathological conditions. Larger scale zero-shot inference tests are necessary to evaluate the generalisability of GAN based CS-MRI methods.

In summary, future research directions on GAN based fast MRI may include more robust training strategies, e.g., combining GAN with genetic algorithm \cite{hao2020annealing}, incorporating edge and texture enhancement \cite{chen2021wavelet}, reducing possible hallucination \cite{zhu2019can,zhu2019lesion}, coupling with explainable AI (XAI) modules \cite{ye2021explainable,yang2021unbox}, and further consideration with MR physics \cite{lv2021pic}.

==> GAN Powered Fast MRI/sections/fundamental_MRI_recon.tex <==
\sloppy

The basis of undersampled MR reconstruction is inferring the missing \textit{k}-space data from the already sampled \textit{k}-space values. For example, in partial Fourier imaging (PFI), 50\% of the \textit{k}-space is acquired. Because the \textit{k}-space is conjugate symmetric, the other missing 50\% is obtained via complex conjugation of the existing 50\%. However, the maximum acceleration is only 2-fold and the reconstructed image exhibits a lower signal-to-noise ratio (SNR) \cite{Hollingsworth2015}.  Another key undersampling technique is parallel imaging (PI). In PI, multiple receiver coils simultaneously collect the \textit{k}-space information of the tissues closest to each coil. However, the acceleration factor is limited by the number and the configuration of the receiver coils \cite{Hollingsworth2015,deshmane_parallel_2012}. Therefore, limits of accelerating MR image acquisition exist for both PI and PFI, bound by the Nyquist-Shannon sampling criteria \cite{Lustig2007}.

Compressed sensing (CS)-based reconstruction circumvents the Nyquist-Shannon sampling criteria and achieves a higher acceleration ratio. CS establishes the model of MR image acquisition as (notations in Table \ref{tab:CS_notation}):
\begin {equation}
    y_u = Ax_t,
\label{eq:CS_acquisition}\end {equation}
where $y_u$ is the undersampled \textit{k}-space signal and $x_t$ is the original fully sampled image. $A$ is an operator defined as: 
\begin{equation}
    A = \Psi \mathcal{F},
\end{equation}
where $\Psi$ is the undersampling mask, a binary matrix denoting which \textit{k}-space locations are sampled and which are not, and $\mathcal{F}$ is the Fourier transform operator. Hence, $\Psi \mathcal{F} x_t$, or $Ax_t$ is equivalent to undersampling the
\textit{k}-space of the putative reconstructed MR image. 

A CS-model infers the underlying full resolution MR image $x_t$ from the collected incomplete \textit{k}-space samples $y_u$ by solving the following optimisation problem \cite{Lustig2007}:
\begin{equation}
    \argmin_{\hat x_u} \frac{\lambda}{2}||y_u-A \hat x_u||_2^2 + R(\hat x_u),
\label{eq:CS_eq}\end{equation}
where $\lambda$ adjusts the contribution of the first term to the optimisation objective and $R(\hat x_u)$ is an image regulariser function.  If this reconstructed image $\hat x_u$ is to match the original image, their undersampled \textit{k}-space results ought to match, as reflected in the first term of Eq \ref{eq:CS_eq}. This reinforces the \textit{k}-space data fidelity of reconstructing the undersampled data.

The second term in Eq \ref{eq:CS_eq} ensures the reconstructed image possesses certain attributes such as smoothness or sparsity, which is required by the theory of CS. 
For example, total variation---an early CS technique---uses the following regulariser term to ensure the underlying image is smooth \cite{Lustig2007,zhang_deep_2020-2}:
\begin{equation}
    \argmin_{\hat x_u} \frac{\lambda}{2}||y_u-A \hat x_u||_2^2 + ||\nabla \hat x_u||_1,
\label{eq:CS_TV}\end{equation}
where $\nabla$ is the gradient operator to minimise the difference between adjacent pixels in the final reconstruction to ensure a smooth texture. To solve Eq \ref{eq:CS_TV}, conjugate gradient descent is employed \cite{Lustig2007}, by updating the reconstructed image with the gradient of Eq \ref{eq:CS_TV} iteratively until convergence.

Another example of CS algorithm is dictionary learning, in which the regulariser function enforces the sparsity of the dictionary representation of each image patch \cite{Ravishankar2011}:
\begin{equation}
    \argmin_{\hat x_u, D, \Gamma} \frac{\lambda}{2}||y_u-A \hat x_u||_2^2 + \sum_{ij}||R_{ij} \hat x_u -Da_{ij}||_2^2,
\label{eq:CS_DL}\end{equation}
where $R_{ij}$ is the image patch extractor, $D$ is the dictionary used to transform the dictionary representation $a_{ij}$ into the image domain, and $\Gamma$ is the set of all dictionary representations $\{a_{ij}\}_{ij}$. This optimisation problem in Eq \ref{eq:CS_DL} is solved by alternating minimisation of the 3 parameter sets iteratively: $\hat x_u$, $D$ and $\Gamma$ collectively. CS algorithms such as TV and dictionary learning repeatedly update the reconstruction to ensure it fulfils \textit{k}-space data fidelity and certain regularisation properties such as sparsity.

From a Bayesian perspective, data fidelity is seen as maximising the conditional probability of observing the undersampled \textit{k}-space data given the reconstructed image. The regulariser term represents the prior expectation of the statistical properties of the final reconstructed image \cite{diamond_unrolled_2017}. By jointly enforcing data fidelity and regulariser constraint, CS reconstruction is equivalent to maximising the posterior probability that the reconstructed image matches the original one given the existing \textit{k}-space samples. This justifies the effectiveness of the CS in reconstructing undersampled MR
images.

% Some Symbol change by Jiahao Huang Apr.28 2021
% Raw \textit{k}-space data --->$y_t$
% Undersampled \textit{k}-space data $y$--->$y_u$
% Image space GT $x_0$--->$x_t$
% Undersampled image space GT --->$x_u$
% Reconstructed MR image $x$--->$\hat x_u$
\begin{table}
\begin{center}
\begin{tabular}{ll}
        \toprule
        \textbf{Symbol} & \textbf{Definition} \\
        \midrule
        $x_t$ & Ground truth MR image \\
        $x_u$ & Undersampled MR image \\
        $\hat x_u$ & Reconstructed MR image \\
        $y_t$ & Ground truth \textit{k}-space signals \\
        $y_u$ & Undersampled \textit{k}-space signals \\
        $\mathcal{F}$ & Fourier transform operator \\
        $\Psi$ & Binary matrix denoting undersampled \textit{k}-space positions  \\
        $A$ & $\Psi \mathcal{F}$  \\
        $R$ & Regularisation function \\
        $\lambda$ & \makecell[l]{ A parameter adjusting the contribution of data \\ fidelity term to the reconstruction loss function} \\
        $\theta$ & Parameters within a convolutional neural network \\
        \bottomrule
\end{tabular}
\end{center}
\caption{Mathematical notations in this book chapter.}
\label{tab:CS_notation}\end{table}
